MaxSAT Evaluation 2019 -- Benchmark: Identifying Security-Critical Cyber-Physical Components in Weighted AND/OR Graphs

This paper presents a MaxSAT benchmark focused on identifying critical nodes in AND/OR graphs. We use AND/OR graphs to model Industrial Control Systems (ICS) as they are able to semantically grasp intricate logical interdependencies among ICS components. However, identifying critical nodes in AND/OR graphs is an NP-complete problem. We address this problem by efficiently transforming the input AND/OR graph-based model into a weighted logical formula that is then used to build and solve a Weighted Partial MaxSAT problem. The benchmark includes 80 cases with AND/OR graphs of different size and composition as well as the optimal cost and solution for each case.

==> sections/dataset1/benchmark1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{table*}[]
%    \hspace{-0.75cm}
    \centering
    \begin{tabular}{@{}|c|c|c|c|c|c|c|c|c|c|@{}}
        \toprule
        \textbf{id} & \textbf{gNodes} & \textbf{gAT} & \textbf{gAND} & \textbf{gOR} & \textbf{tsVars} & \textbf{tsClauses} & \textbf{cost} & \textbf{time} & \textbf{solution}                                                                                                                               \\ \midrule
        1           & 5000            & 3977         & 512           & 512          & 8978            & 23981              & 2             & 1163          & [(14:2)]                                                                                                                                   \\ \midrule
        2           & 5000            & 3967         & 529           & 505          & 8968            & 23971              & 16            & 1264          & [(2:16)]                                                                                                                                   \\ \midrule
        3           & 5000            & 3984         & 515           & 502          & 8985            & 23988              & 2             & 920           & [(98:2)]                                                                                                                                   \\ \midrule
        4           & 5000            & 4008         & 461           & 532          & 9009            & 24012              & 8             & 919           & [(8:1),(961:7)]                                                                                                                            \\ \midrule
        5           & 5000            & 3990         & 510           & 501          & 8991            & 23994              & 1             & 930           & [(4057:1)]                                                                                                                                 \\ \midrule
        6           & 5000            & 4002         & 486           & 513          & 9003            & 24006              & 5             & 946           & [(788:3),(8431:2)]                                                                                                                         \\ \midrule
        7           & 5000            & 4026         & 477           & 498          & 9027            & 24030              & 20            & 920           & [(8:1),(759:12),(6706:3),(6860:1),(7304:3)]                                                                                                \\ \midrule
        8           & 5000            & 3996         & 518           & 487          & 8997            & 24000              & 6             & 894           & [(4:6)]                                                                                                                                    \\ \midrule
        9           & 5000            & 4046         & 488           & 467          & 9047            & 24050              & 5             & 904           & [(3177:5)]                                                                                                                                 \\ \midrule
        10          & 5000            & 4026         & 493           & 482          & 9027            & 24030              & 5             & 887           & [(4029:4),(5503:1)]                                                                                                                        \\ \midrule
        11          & 5000            & 3029         & 979           & 993          & 8030            & 23033              & 31            & 880           & [(1258:30),(2189:1)]                                                                                                                       \\ \midrule
        12          & 5000            & 2998         & 1012          & 991          & 7999            & 23002              & 68            & 935           & [(920:2),(1128:3),(1324:9),(1926:3),(2690:13),(2773:35),(3441:3)]                                                                          \\ \midrule
        13          & 5000            & 3021         & 1008          & 972          & 8022            & 23025              & 2             & 879           & [(300:2)]                                                                                                                                  \\ \midrule
        14          & 5000            & 2986         & 1020          & 995          & 7987            & 22990              & 46            & 956           & [(1027:12),(3624:3),(3778:17),(6453:2),(6496:4),(6544:8)]                                                                                  \\ \midrule
        %15          & 5000            & 3014         & 1006          & 981          & 8015            & 23018              & 152           & 1889          & [(5:1),(2930:5),(3245:7),(3434:34),(3925:17),(4158:14),(4457:34),(6307:19),(7048:5),(7177:2),(7186:1),(7191:7),(7337:1),(7367:1),(7570:4)] \\ \midrule
        15          & 5000            & 3014         & 1006          & 981          & 8015            & 23018              & 152           & 1889          & [(5:1),(2930:5),(3245:7),(3434:34),(3925:17),(4158:14),\\
            &             &          &           &           &             &               &            &          &   (4457:34), (6307:19),(7048:5),(7177:2),(7186:1), \\
            &             &          &           &           &             &               &            &          &            (7191:7),(7337:1),(7367:1),(7570:4)] \\ \midrule
        16          & 5000            & 3030         & 990           & 981          & 8031            & 23034              & 12            & 859           & [(3:12)]                                                                                                                                   \\ \midrule
        17          & 5000            & 3015         & 1034          & 952          & 8016            & 23019              & 3             & 867           & [(4:2),(7561:1)]                                                                                                                           \\ \midrule
        18          & 5000            & 3008         & 956           & 1037         & 8009            & 23012              & 22            & 877           & [(2:19),(6253:3)]                                                                                                                          \\ \midrule
        19          & 5000            & 3031         & 970           & 1000         & 8032            & 23035              & 8             & 865           & [(5444:8)]                                                                                                                                 \\ \midrule
        20          & 5000            & 3033         & 972           & 996          & 8034            & 23037              & 13            & 870           & [(2:13)]                                                                                                                                   \\ \midrule
        21          & 10000           & 7983         & 1017          & 1001         & 17984           & 47987              & 1             & 1126          & [(16139:1)]                                                                                                                                \\ \midrule
        22          & 10000           & 8026         & 996           & 979          & 18027           & 48030              & 13            & 1313          & [(2:13)]                                                                                                                                   \\ \midrule
        23          & 10000           & 8024         & 991           & 986          & 18025           & 48028              & 12            & 1310          & [(24:1),(1580:1),(2201:2),(9663:3),(14360:5)]                                                                                              \\ \midrule
        24          & 10000           & 8058         & 974           & 969          & 18059           & 48062              & 14            & 1184          & [(5:9),(12130:2),(12207:2),(12422:1)]                                                                                                      \\ \midrule
        25          & 10000           & 8026         & 989           & 986          & 18027           & 48030              & 7             & 1459          & [(9009:3),(12030:4)]                                                                                                                       \\ \midrule
        26          & 10000           & 7984         & 1003          & 1014         & 17985           & 47988              & 12            & 1309          & [(7:9),(17023:1),(17074:2)]                                                                                                                \\ \midrule
        %27          & 10000           & 8051         & 939           & 1011         & 18052           & 48055              & 50            & 6248          & [(1997:4),(2744:9),(3398:17),(5610:6),(6304:1),(11315:1),(11771:4),(14136:1),(16399:4),(16831:3)]                                          \\ \midrule
    
        27          & 10000           & 8051         & 939           & 1011         & 18052           & 48055              & 50            & 6248          & [(1997:4),(2744:9),(3398:17),(5610:6),(6304:1),(11315:1),(11771:4), \\
                   &             &          &           &           &             &               &            &          &  (14136:1),(16399:4),(16831:3)]     \\ \midrule
        28          & 10000           & 7998         & 995           & 1008         & 17999           & 48002              & 3             & 1141          & [(2:3)]                                                                                                                                    \\ \midrule
        29          & 10000           & 8095         & 972           & 934          & 18096           & 48099              & 10            & 1224          & [(8330:4),(11696:5),(13881:1)]                                                                                                             \\ \midrule
        30          & 10000           & 8022         & 987           & 992          & 18023           & 48026              & 2             & 1178          & [(2:2)]                                                                                                                                    \\ \midrule
        31          & 10000           & 6013         & 1991          & 1997         & 16014           & 46017              & 49            & 1275          & [(4:32),(4857:17)]                                                                                                                         \\ \midrule
        32          & 10000           & 5981         & 2039          & 1981         & 15982           & 45985              & 7             & 1098          & [(5929:5),(6199:2)]                                                                                                                        \\ \midrule
        33          & 10000           & 6023         & 1957          & 2021         & 16024           & 46027              & 12            & 1127          & [(3:12)]                                                                                                                                   \\ \midrule
        %34          & 10000           & 6015         & 2021          & 1965         & 16016           & 46019              & 60            & 1247          & [(5641:17),(5858:3),(5969:16),(5997:6),(6025:6),(6033:3),(6133:2),(9790:2),(11731:5)]                                                      \\ \midrule
        34          & 10000           & 6015         & 2021          & 1965         & 16016           & 46019              & 60            & 1247          & [(5641:17),(5858:3),(5969:16),(5997:6),(6025:6),(6033:3), \\
                           &             &          &           &           &             &               &            &          &  (6133:2),(9790:2),(11731:5)]           \\ \midrule
        35          & 10000           & 5953         & 1975          & 2073         & 15954           & 45957              & 24            & 1071          & [(2:24)]                                                                                                                                   \\ \midrule
        36          & 10000           & 6030         & 2034          & 1937         & 16031           & 46034              & 36            & 1279          & [(12930:22),(15804:2),(15947:12)]                                                                                                          \\ \midrule
        37          & 10000           & 6008         & 1996          & 1997         & 16009           & 46012              & 3             & 1092          & [(13780:3)]                                                                                                                                \\ \midrule
        38          & 10000           & 6054         & 1963          & 1984         & 16055           & 46058              & 1             & 1111          & [(3447:1)]                                                                                                                                 \\ \midrule
        39          & 10000           & 6015         & 1977          & 2009         & 16016           & 46019              & 27            & 1194          & [(2391:27)]                                                                                                                                \\ \midrule
        40          & 10000           & 6042         & 1967          & 1992         & 16043           & 46046              & 73            & 2607          & [(2820:1),(7720:3),(8418:14),(8586:2),(10093:46),(12532:7)]                                                                                \\ \bottomrule
    \end{tabular}
    \vspace{0.5cm}
    \caption{Benchmark description - Cases 1 to 40}
    \label{tab:benchmark-part1}
\end{table*}

==> sections/dataset1/benchmark2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\begin{tabular}{@{}|c|c|c|c|c|c|c|c|c|c|@{}}
\toprule
\textbf{id} & \textbf{gNodes} & \textbf{gAT} & \textbf{gAND} & \textbf{gOR} & \textbf{tsVars} & \textbf{tsClauses} & \textbf{cost} & \textbf{time} & \textbf{solution} \\ \midrule
41 & 15000 & 12090 & 1443 & 1468 & 27091 & 72094 & 16 & 3024 & [(97:8),(6443:8)] \\ \midrule
42 & 15000 & 11973 & 1517 & 1511 & 26974 & 71977 & 3 & 2139 & [(14702:3)] \\ \midrule
43 & 15000 & 12004 & 1529 & 1468 & 27005 & 72008 & 2 & 1511 & [(1021:1),(22132:1)] \\ \midrule
44 & 15000 & 11969 & 1517 & 1515 & 26970 & 71973 & 18 & 10965 & [(2:18)] \\ \midrule
45 & 15000 & 12123 & 1457 & 1421 & 27124 & 72127 & 5 & 1576 & [(2350:1),(2665:1),(3626:3)] \\ \midrule
46 & 15000 & 11969 & 1480 & 1552 & 26970 & 71973 & 5 & 1564 & [(13:4),(25198:1)] \\ \midrule
47 & 15000 & 11949 & 1490 & 1562 & 26950 & 71953 & 9 & 1605 & [(58:1),(3272:6),(6793:2)] \\ \midrule
48 & 15000 & 11982 & 1542 & 1477 & 26983 & 71986 & 18 & 2863 & [(5:18)] \\ \midrule
49 & 15000 & 12015 & 1486 & 1500 & 27016 & 72019 & 3 & 1511 & [(2649:1),(6731:2)] \\ \midrule
50 & 15000 & 11980 & 1496 & 1525 & 26981 & 71984 & 1 & 1627 & [(1853:1)] \\ \midrule
51 & 15000 & 9043 & 2893 & 3065 & 24044 & 69047 & 11 & 1423 & [(22630:2),(22728:9)] \\ \midrule
52 & 15000 & 9036 & 2976 & 2989 & 24037 & 69040 & 123 & 9571 & [(10932:44),(13135:5),(15118:5),(15681:3),(15695:66)] \\ \midrule
53 & 15000 & 9046 & 2938 & 3017 & 24047 & 69050 & 14 & 1182 & [(3:6),(14013:8)] \\ \midrule
54 & 15000 & 9015 & 3028 & 2958 & 24016 & 69019 & 47 & 1502 & [(3:42),(11757:2),(13221:3)] \\ \midrule
55 & 15000 & 8987 & 3035 & 2979 & 23988 & 68991 & 8 & 1208 & [(17563:3),(17567:5)] \\ \midrule
56 & 15000 & 9015 & 3002 & 2984 & 24016 & 69019 & 1 & 1483 & [(15321:1)] \\ \midrule
%57 & 15000 & 9099 & 2966 & 2936 & 24100 & 69103 & 80 & 5040 & [(3352:8),(3770:4),(8682:5),(10152:8),(10159:3),(10239:1),(10468:3),(18507:6),(18555:8),(18573:2),(18628:8),(18753:14),(19274:5),(22843:2),(23171:3)] \\ \midrule
57 & 15000 & 9099 & 2966 & 2936 & 24100 & 69103 & 80 & 5040 & [(3352:8),(3770:4),(8682:5),(10152:8),(10159:3),(10239:1),\\
     &             &          &           &           &             &               &            &          &  (10468:3), (18507:6),(18555:8),(18573:2),(18628:8),(18753:14),\\
     &             &          &           &           &             &               &            &          &  (19274:5),(22843:2),(23171:3)] \\ \midrule
58 & 15000 & 9011 & 2943 & 3047 & 24012 & 69015 & 4 & 1152 & [(18688:2),(19011:2)] \\ \midrule
59 & 15000 & 9035 & 2998 & 2968 & 24036 & 69039 & 53 & 10802 & [(2:53)] \\ \midrule
60 & 15000 & 9013 & 3066 & 2922 & 24014 & 69017 & 14 & 1264 & [(11895:1),(12533:3),(12590:3),(16787:2),(23583:5)] \\ \midrule
61 & 20000 & 16004 & 1975 & 2022 & 36005 & 96008 & 1 & 1637 & [(16475:1)] \\ \midrule
62 & 20000 & 15977 & 1958 & 2066 & 35978 & 95981 & 3 & 1686 & [(34706:3)] \\ \midrule
63 & 20000 & 16007 & 2071 & 1923 & 36008 & 96011 & 1 & 2040 & [(32144:1)] \\ \midrule
64 & 20000 & 16067 & 1978 & 1956 & 36068 & 96071 & 1 & 1572 & [(35189:1)] \\ \midrule
65 & 20000 & 15999 & 1990 & 2012 & 36000 & 96003 & 2 & 1873 & [(12825:2)] \\ \midrule
66 & 20000 & 15947 & 2037 & 2017 & 35948 & 95951 & 4 & 2074 & [(3:4)] \\ \midrule
67 & 20000 & 16019 & 1992 & 1990 & 36020 & 96023 & 7 & 2153 & [(6:3),(20228:4)] \\ \midrule
68 & 20000 & 15976 & 2036 & 1989 & 35977 & 95980 & 5 & 1492 & [(7:2),(17657:2),(24220:1)] \\ \midrule
69 & 20000 & 16019 & 1997 & 1985 & 36020 & 96023 & 9 & 2545 & [(3:9)] \\ \midrule
70 & 20000 & 16052 & 1909 & 2040 & 36053 & 96056 & 2 & 2031 & [(29145:2)] \\ \midrule
71 & 20000 & 12037 & 4033 & 3931 & 32038 & 92041 & 2 & 1847 & [(21278:2)] \\ \midrule
%72 & 20000 & 11977 & 3997 & 4027 & 31978 & 91981 & 373 & 12887 & [(1172:17),(11919:5),(12728:2),(1295:1),(13840:2),(14081:4),(14453:22),(15461:5),(16291:13),(17369:3),(18459:20),(19920:1),(19925:4),(20651:2),(20789:37),(20929:9),(21080:41),(22175:7),(22642:1),(22804:27),(22806:12),(22809:3),(22818:26),(22829:6),(22852:31),(23065:7),(28543:65)] \\ \midrule
72 & 20000 & 11977 & 3997 & 4027 & 31978 & 91981 & 373 & 12887 & [(1172:17),(11919:5),(12728:2),(1295:1),(13840:2),(14081:4),\\
     &             &          &           &           &             &               &            &          & (14453:22), (15461:5),(16291:13),(17369:3),(18459:20),(19920:1),\\
     &             &          &           &           &             &               &            &          & (19925:4),(20651:2), (20789:37),(20929:9),(21080:41),(22175:7), \\
          &             &          &           &           &             &               &            &          & (22642:1),(22804:27),(22806:12),(22809:3),(22818:26),(22829:6),\\
     &             &          &           &           &             &               &            &          &  (22852:31),(23065:7),(28543:65)] \\ \midrule
73 & 20000 & 12037 & 3999 & 3965 & 32038 & 92041 & 3 & 1513 & [(22359:2),(30489:1)] \\ \midrule
74 & 20000 & 12004 & 3980 & 4017 & 32005 & 92008 & 1 & 1434 & [(2:1)] \\ \midrule
75 & 20000 & 12059 & 3930 & 4012 & 32060 & 92063 & 28 & 3071 & [(2:18),(26845:10)] \\ \midrule
76 & 20000 & 12094 & 3858 & 4049 & 32095 & 92098 & 2 & 1772 & [(6431:2)] \\ \midrule
77 & 20000 & 12000 & 4014 & 3987 & 32001 & 92004 & 3 & 1474 & [(27418:3)] \\ \midrule
78 & 20000 & 12110 & 3940 & 3951 & 32111 & 92114 & 4 & 1665 & [(4:4)] \\ \midrule
%79 & 20000 & 12036 & 4012 & 3953 & 32037 & 92040 & 71 & 1600 & [(2:9),(14499:3),(17840:14),(19998:32),(28910:2),(29045:9),(29937:2)] \\ \midrule
79 & 20000 & 12036 & 4012 & 3953 & 32037 & 92040 & 71 & 1600 & [(2:9),(14499:3),(17840:14),(19998:32),(28910:2),\\
     &             &          &           &           &             &               &            &          &  (29045:9),(29937:2)] \\ \midrule
80 & 20000 & 12035 & 4055 & 3911 & 32036 & 92039 & 8 & 1688 & [(13697:8)] \\ \bottomrule
\end{tabular}
 \vspace{0.5cm}
\caption{Benchmark description - Cases 41 to 80}
\label{tab:benchmark-part2}
\end{table*}
